The Complexity of Shake Slice Knots

We define a notion of complexity for shake-slice knots which is analogous to the definition of complexity for h-cobordisms studied by Morgan-Szab\'o. We prove that for each framing $n \ne 0$ and complexity $c \ge 0$, there is an $n$-shake-slice knot with complexity at least $c$. Our construction makes use of dualizable patterns, and we include a crash course in their properties. We bound complexity by studying the behavior of the classical knot signature and the Levine-Tristram signature of a knot under the operation of twisting algebraically-one strands.

==> The complexity of shake slice knots/commands.tex <==
% Master commands file
% Dependencies: none

% Text
\newcommand{\OneHalf}{{\textstyle\frac{1}{2}}}
\newcommand{\OneQuart}{{\textstyle\frac{1}{4}}}

% environments
\newenvironment{idea}{\vspace{5mm}\par\color{blue} \indent IDEA:\hspace{5mm}}{\par \vspace{5mm}}

% Hyphenation.
\hyphenation{Thurs-ton}
\hyphenation{mo-no-poles}
\hyphenation{sur-ger-y}

%-------------------------------------------------------------------------------

% Common Fractions

\newcommand{\invs}{^{-1}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\third}{\frac{1}{3}}
\newcommand{\quarter}{\frac{1}{4}}
\newcommand{\fifth}{\frac{1}{5}}
\newcommand{\sixth}{\frac{1}{6}}
\newcommand{\eighth}{\frac{1}{8}}



% Pairs of openings and closures
\newcommand{\set}[1]{\mathchoice%
  {\left\lbrace #1 \right\rbrace}%
  {\lbrace #1 \rbrace}%
  {\lbrace #1 \rbrace}%
  {\lbrace #1 \rbrace}%
}
\newcommand{\setc}[2]{\mathchoice%
  {\left\lbrace #1 \, \middle\vert \, #2 \right\rbrace}%
  {\lbrace #1 \, \vert \, #2 \rbrace}%
  {\lbrace #1 \, \vert \, #2 \rbrace}%
  {\lbrace #1 \, \vert \, #2 \rbrace}%
%  {\left\lbrace #1 \, \colon \, #2 \right\rbrace}%
%  {\lbrace #1 \, \colon \, #2 \rbrace}%
%  {\lbrace #1 \, \colon \, #2 \rbrace}%
%  {\lbrace #1 \, \colon \, #2 \rbrace}%
}
\newcommand{\paren}[1]{\mathchoice%
  {\left( #1 \right)}%
  {( #1 )}%
  {( #1 )}%
  {( #1 )}%
}
\newcommand{\brac}[1]{\mathchoice%
  {\left[ #1 \right]}%
  {[ #1 ]}%
  {[ #1 ]}%
  {[ #1 ]}%
}
\newcommand{\abs}[1]{\mathchoice%
  {\left\lvert #1 \right\rvert}%
  {\lvert #1 \rvert}%
  {\lvert #1 \rvert}%
  {\lvert #1 \rvert}%
}
\newcommand{\norm}[1]{\mathchoice%
  {\left\lVert #1 \right\rVert}%
  {\lVert #1 \rVert}%
  {\lVert #1 \rVert}%
  {\lVert #1 \rVert}%
}
\newcommand{\ang}[1]{\mathchoice%
  {\left\langle #1 \right\rangle}%
  {\langle #1 \rangle}%
  {\langle #1 \rangle}%
  {\langle #1 \rangle}%
}

% Synonyms for symbols
\renewcommand{\bar}{\overline}
\renewcommand{\hat}{\widehat}
\newcommand{\dual}{^*}
\newcommand{\pound}{_{\#}}
\newcommand{\ppp}{^{\prime\prime\prime}}
\newcommand{\pp}{^{\prime\prime}}        %extra {} make sure the two primes play nicely with the ^ operator. 
\newcommand{\eps}{\epsilon}                  % mathord
\newcommand{\veps}{\varepsilon}              % mathord
%\renewcommand{\phi}{\varphi}                 % mathord
\newcommand{\vphi}{\varphi}                  % mathord
\newcommand{\eset}{\varnothing}             % mathord
%\newcommand{\eset}{\emptyset}                % mathord

\newcommand{\dirsum}{\oplus}                 % mathbin
\newcommand{\bigdirsum}{\bigoplus}           % mathop
\newcommand{\tensor}{\otimes}                % mathbin
\newcommand{\bigtensor}{\bigotimes}          % mathop
\newcommand{\union}{\cup}                    % mathbin
\newcommand{\bigunion}{\bigcup}              % mathop
\newcommand{\intersect}{\cap}                % mathbin
\newcommand{\bigintersect}{\bigcap}          % mathop

\newcommand{\of}{\circ}                    % mathbin
\newcommand{\cross}{\times}                  % mathbin

\newcommand{\isom}{\cong}                    % mathrel
\newcommand{\qisom}{\simeq}                  % mathrel
\newcommand{\nisom}{\ncong}                  % mathrel
\newcommand{\nqisom}{\not\simeq}             % mathrel
\newcommand{\superset}{\supset}              % mathrel
\newcommand{\contains}{\ni}                  % mathrel
\newcommand{\into}{\hookrightarrow}

% Special sets
\newcommand{\numset}[1]{\mathbb{#1}}
\newcommand{\one}{\mathbb{1}}
\newcommand{\N}{{\numset{Z}_{>0}}}
\newcommand{\Z}{\numset{Z}}
\newcommand{\Zpos}{\Z_{\geq 0}}
\newcommand{\Q}{\numset{Q}}
\newcommand{\R}{\numset{R}}
\newcommand{\C}{\numset{C}}
\newcommand{\F}[1]{\numset{F}_{#1}}
\newcommand{\FF}{\numset{F}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\Tminus}{\mathcal{T}^{-}}
\newcommand{\Tplus}{\mathcal{T}^{+}}
\newcommand{\cycgrp}[1]{\Z / #1 \Z}
\newcommand{\field}[1]{\mathbf{#1}}
\renewcommand{\j}{\field{j}}
\renewcommand{\k}{\field{k}}

% Punctuation
%\newcommand{\co}{\colon}
%\newcommand{\semico}{;\penalty 300}
\newcommand{\scolon}{; \penalty 300}

% Common operators
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\nll}{null}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Coker}{Coker}
\DeclareMathOperator{\im}{Im} % Image
\DeclareMathOperator{\homgy}{H} % Homology
\DeclareMathOperator{\Hom}{Hom} % Homomorphism
\DeclareMathOperator{\Cone}{Cone}
\DeclareMathOperator{\rk}{rk} % Rank
\DeclareMathOperator{\Hochsch}{HH} % Hochschild homology
\newcommand{\MCG}{\mathit{MCG}} % Mapping class group
\DeclareMathOperator{\Neg}{neg}
\DeclareMathOperator{\double}{double}

% Matrix groups
\newcommand{\matrixgrp}[1]{\mathrm{#1}}
\newcommand{\GL}{\matrixgrp{GL}}
\newcommand{\SL}{\matrixgrp{SL}}
\newcommand{\SO}{\matrixgrp{SO}}
\newcommand{\SU}{\matrixgrp{SU}}
\newcommand{\Sp}{\matrixgrp{Sp}}
\newcommand{\ISO}{\matrixgrp{ISO}}
\newcommand{\Spin}{\matrixgrp{Spin}}
\newcommand{\Spinc}{Spin\textsuperscript{c} }

% Lie algebras
\newcommand{\fsl}{\mathfrak{sl}}
\newcommand{\sltwo}{\fsl_2}
\newcommand{\fg}{\mathfrak g}
\newcommand{\fgl}{\mathfrak{gl}}
\newcommand{\gloneone}{\fgl_{1|1}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\ft}{\mathfrak{t}}

% Basic topology
\newcommand{\homeo}{\approx}
\newcommand{\homeob}{\approx_\partial}
\newcommand{\diffeo}{\cong}
\newcommand{\torus}{\mathbb{T}}
\newcommand{\boundary}{\partial} % mathord
\newcommand{\connsum}{\mathbin{\#}} % Originally mathord
\newcommand{\bigconnsum}{\mathop{\mathchoice%
    {\vcenter{\hbox{\LARGE $\#$}}}
    {\vcenter{\hbox{\large $\#$}}}
    {\vcenter{\hbox{\footnotesize $\#$}}}
    {\vcenter{\hbox{\scriptsize $\#$}}}
  }}
\newcommand{\bdysum}{\mathbin{\natural}} % Originally mathord
\newcommand{\bigbdysum}{\mathop{\mathchoice%
    {\vcenter{\hbox{\LARGE $\natural$}}}
    {\vcenter{\hbox{\large $\natural$}}}
    {\vcenter{\hbox{\footnotesize $\natural$}}}
    {\vcenter{\hbox{\scriptsize $\natural$}}}
  }}
\DeclareMathOperator{\Sym}{Sym}
\newcommand{\unknot}{\mathord{\bigcirc}} % Originally mathbin
\newcommand{\quasialt}{\mathcal{Q}} % Quasi-alternating links
\newcommand{\QHS}{{\Q}\mathit{HS}^3}
\newcommand{\ZHS}{{\Z}\mathit{HS}^3}
\newcommand{\nbhd}[1]{\nu (#1)}

\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\core}{core}
\DeclareMathOperator{\cocore}{cocore}
% Signature
\DeclareMathOperator{\sign}{sign}

%Knot Theory
\DeclareMathOperator{\whitehead}{Wh}
\DeclareMathOperator{\shake}{Sh}
\DeclareMathOperator{\writhe}{writhe}
\DeclareMathOperator{\arf}{Arf}

% Spheres, disks, ...
\newcommand{\sphere}[1]{{S}^{#1}}
\newcommand{\disk}[1]{{D}^{#1}}
\newcommand{\ball}[1]{{B}^{#1}}
\newcommand{\interval}{{I}}
\newcommand{\RP}[1]{\mathbb{RP}^{#1}}
\newcommand{\CP}[1]{\mathbb{CP}^{#1}}
\newcommand{\CPbar}[1]{\overline{\mathbb{CP}}^{#1}}

\renewcommand{\SS}[2]{{S}^{#1}\times{S}^{#2}}
\newcommand{\SD}[2]{{S}^{#1}\times{D}^{#2}}
\newcommand{\DS}[2]{{D}^{#1}\times{S}^{#2}}
\newcommand{\DD}[2]{{D}^{#1}\times{D}^{#2}}
\newcommand{\SB}[2]{{S}^{#1}\times{B}^{#2}}
\newcommand{\BS}[2]{{B}^{#1}\times{S}^{#2}}
\newcommand{\BB}[2]{{B}^{#1}\times{B}^{#2}}

\newcommand{\laurent}{\ZZ[t, t^{-1}]}
% Blanchfield
\newcommand{\Bl}{\operatorname{Bl}}



% Special for this context

\DeclareMathOperator{\genus}{genus}

\newcommand{\SPC}{SPC4 }


==> The complexity of shake slice knots/macros.tex <==
\makeatletter
\g@addto@macro\@floatboxreset\centering
\makeatother

\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother

\def\mathcenter#1{%
  \vcenter{\hbox{$#1$}}%
}

\allowdisplaybreaks[4]

\addto\extrasamerican{%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \def\subsubsectionautorefname{Section}%
}

\let\fullref\autoref

\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\theoremstyle{definition}
\newtheorem*{convention}{Conventions}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{question}{Question}[section]

\makeatletter
\let\c@conjecture=\c@theorem
\let\c@corollary=\c@theorem
\let\c@observation=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@definition=\c@theorem
\let\c@example=\c@theorem
\let\c@remark=\c@theorem
\let\c@question=\c@theorem
\let\c@equation\c@theorem
\makeatother

\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}
\makeautorefname{theorem}{Theorem}%
\makeautorefname{conjecture}{Conjecture}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{observation}{Observation}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{definition}{Definition}%
\makeautorefname{example}{Example}%
\makeautorefname{remark}{Remark}%
\makeautorefname{question}{Question}%

\numberwithin{equation}{section}

\newcommand*{\Alphabet}{ABCDEFGHIJKLMNOPQRSTUVWXYZ1234567890}
\newcommand*{\alphabet}{abcdefghijklmnopqrstuvwxyz1234567890}
\newlength\fcaph
\newlength\fdesc
\newlength\factualfontsize
\settoheight{\fcaph}{\footnotesize \Alphabet}
\settodepth{\fdesc}{\footnotesize \Alphabet \alphabet}
\setlength{\factualfontsize}{\dimexpr\fcaph+\fdesc\relax}

% Comments
\numberwithin{equation}{section}
\newcounter{commentcounter}
\newcommand{\commentb}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by B.)}:
	{\textcolor{blue}{#1}} }
\newcommand{\commentc}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by C.)}:
	{\textcolor{purple}{#1}} }
\newcommand{\commentm}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by M.)}:
	{\textcolor{orange}{#1}} }
	
	
\newcommand{\TODO}{\textcolor{magenta}{TODO}}

==> The complexity of shake slice knots/mathabx.tex <==

\makeatletter
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}

\let\widecheck\@undefined
\let\widebar\@undefined
\DeclareMathAccent{\widecheck}{\mathord}{mathx}{"71}
\DeclareMathAccent{\widebar}{\mathord}{mathx}{"73}
\makeatother



==> The complexity of shake slice knots/mnsymbol.tex <==

\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother



==> The complexity of shake slice knots/stmry.tex <==

\makeatletter
\DeclareSymbolFont{stmry}{U}{stmry}{m}{n}
\SetSymbolFont{stmry}{bold}{U}{stmry}{b}{n}

\let\llbracket\@undefined
\let\rrbracket\@undefined
\DeclareMathDelimiter{\llbracket}{\mathopen}%
                     {stmry}{"4A}{stmry}{"71}
\DeclareMathDelimiter{\rrbracket}{\mathclose}%
                     {stmry}{"4B}{stmry}{"79}
\makeatother



==> macros.tex <==
\makeatletter
\g@addto@macro\@floatboxreset\centering
\makeatother

\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother

\def\mathcenter#1{%
  \vcenter{\hbox{$#1$}}%
}

\allowdisplaybreaks[4]

\addto\extrasamerican{%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \def\subsubsectionautorefname{Section}%
}

\let\fullref\autoref

\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\theoremstyle{definition}
\newtheorem*{convention}{Conventions}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{question}{Question}[section]

\makeatletter
\let\c@conjecture=\c@theorem
\let\c@corollary=\c@theorem
\let\c@observation=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@definition=\c@theorem
\let\c@example=\c@theorem
\let\c@remark=\c@theorem
\let\c@question=\c@theorem
\let\c@equation\c@theorem
\makeatother

\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}
\makeautorefname{theorem}{Theorem}%
\makeautorefname{conjecture}{Conjecture}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{observation}{Observation}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{definition}{Definition}%
\makeautorefname{example}{Example}%
\makeautorefname{remark}{Remark}%
\makeautorefname{question}{Question}%

\numberwithin{equation}{section}

\newcommand*{\Alphabet}{ABCDEFGHIJKLMNOPQRSTUVWXYZ1234567890}
\newcommand*{\alphabet}{abcdefghijklmnopqrstuvwxyz1234567890}
\newlength\fcaph
\newlength\fdesc
\newlength\factualfontsize
\settoheight{\fcaph}{\footnotesize \Alphabet}
\settodepth{\fdesc}{\footnotesize \Alphabet \alphabet}
\setlength{\factualfontsize}{\dimexpr\fcaph+\fdesc\relax}

% Comments
\numberwithin{equation}{section}
\newcounter{commentcounter}
\newcommand{\commentb}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by B.)}:
	{\textcolor{blue}{#1}} }
\newcommand{\commentc}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by C.)}:
	{\textcolor{purple}{#1}} }
\newcommand{\commentm}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by M.)}:
	{\textcolor{orange}{#1}} }
	
	
\newcommand{\TODO}{\textcolor{magenta}{TODO}}

==> mnsymbol.tex <==

\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother


